Feynman-Kac Correctors in Diffusion: Annealing, Guidance, and Product of Experts

While score-based generative models are the model of choice across diverse domains, there are limited tools available for controlling inference-time behavior in a principled manner, e.g. for composing multiple pretrained models. Existing classifier-free guidance methods use a simple heuristic to mix conditional and unconditional scores to approximately sample from conditional distributions. However, such methods do not approximate the intermediate distributions, necessitating additional `corrector' steps. In this work, we provide an efficient and principled method for sampling from a sequence of annealed, geometric-averaged, or product distributions derived from pretrained score-based models. We derive a weighted simulation scheme which we call Feynman-Kac Correctors (FKCs) based on the celebrated Feynman-Kac formula by carefully accounting for terms in the appropriate partial differential equations (PDEs). To simulate these PDEs, we propose Sequential Monte Carlo (SMC) resampling algorithms that leverage inference-time scaling to improve sampling quality. We empirically demonstrate the utility of our methods by proposing amortized sampling via inference-time temperature annealing, improving multi-objective molecule generation using pretrained models, and improving classifier-free guidance for text-to-image generation. Our code is available at https://github.com/martaskrt/fkc-diffusion.

==> old_derivations/geometric_mixtures.tex <==

\subsection{Geometric Mixtures}
Consider two score functions $\nabla \log \pone_{1-\tau}, \nabla \log \ptwo_{1-\tau}$ trained to reverse the same noising dynamics with drift $\bref_t$ and diffusion $\sigma_t$,
\begin{align}
\partial_\tau \pone_{1-\tau} &= - \langle \nabla, \pone_{1-\tau} \left(-\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pone_{1-\tau} \right) \rangle + \frac{\sigma_{1-\tau}^2}{2}\Delta \pone_{1-\tau} \\
\partial_\tau \ptwo_{1-\tau} &= - \langle \nabla, \ptwo_{1-\tau} \left(-\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \ptwo_{1-\tau} \right) \rangle + \frac{\sigma_{1-\tau}^2}{2}\Delta \ptwo_{1-\tau} 
\end{align}
We now want to sample from the scaled geometric mixture
\begin{align}
\pgeo_{1-\tau}(x) = \frac{1}{\cZ} \pone_{1-\tau}(x)^{\lambda (1-\gamma)} \ptwo_{1-\tau}(x)^{\lambda \gamma}\label{eq:tgt}
\end{align}
We have two considerations when constructing a weighted SDE, which we will simulate to approximate \cref{eq:tgt}:
\begin{itemize}
    \item \textbf{Choice of Proposal:}  i.e. the drift of the SDE we simulate
    \item \textbf{Computational Cost for the Weights:}  i.e. we would like to avoid Laplacians of score functions or divergences of neural-network vector fields
\end{itemize}
We will find that simulating the score function $\nabla \log \pgeo_{1-\tau}(x) = \lambda(1-\gamma) \nabla \log \pone_{1-\tau} + \lambda \gamma \nabla \log \ptwo_{1-\tau}$ yields easy-to-calculate weights.  Further, we expect it to be a good, training-free proposal since it incorporates both score functions.
\begin{mybox}
\begin{proposition} \label{prop:fk_sim}
The target $\pgeo_{1-\tau}$ in \cref{eq:tgt} satisfies the following PDE,
%\small 
    \begin{align}
   % \partial_\tau  \pgeo_{1-\tau}  &= -\left\langle \nabla,\pgeo_{1-\tau}\left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) \right\rangle + \frac{\sigma_{1-\tau}^2}{2} \Delta \pgeo_{1-\tau} \\
   % &\phantom{=} + \pgeo_{1-\tau}\left( (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} + \left(1-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2  + \lambda \gamma (1-\gamma) \sigma_{1-\tau}^2\langle\nabla \log \pone_{1-\tau}, \nabla \log \ptwo_{1-\tau} \rangle\right) \nonumber \\
      \partial_\tau  \pgeo_{1-\tau}  &= -\left\langle \nabla,\pgeo_{1-\tau}\left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) \right\rangle + \frac{\sigma_{1-\tau}^2}{2} \Delta \pgeo_{1-\tau} \\
   &\phantom{=} + \pgeo_{1-\tau}\Bigg(  (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} +
\left({1}-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2 \nonumber \\
 &\phantom{= + \pgeo_{1-\tau}\Bigg(}
 - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2  \Bigg) \nonumber \\
   &\phantom{=} - \pgeo_{1-\tau} ~\mathbb{E}_{\pgeo_{1-\tau}}\left[ \left( \cdot \right) \right] \nonumber
\end{align}
\normalsize
which suggests simulation using the following weighted SDE
\begin{align}
dx_\tau &= \left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) d\tau + \sigma_{1-\tau} \rev{dW_\tau}\label{eq:weighted_sde} \\
d\log w_\tau &= \Bigg(  (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} +
\left({1}-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2 \\
&\phantom{\Bigg(====} 
 - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 
\Bigg) d\tau \nonumber
\end{align}
\end{proposition}
\end{mybox}
See proof in \cref{sec:proof} below.
    \begin{mybox}
\begin{example}[Product Distribution]
    Let $\gamma = \sfrac{1}{2}$ to obtain equal exponential weights on $\pone(x)^{\frac{1}{2}}$, $\ptwo(x)^{\frac{1}{2}}$, with $\lambda= 2$ to sample from the product distribution $\pgeo_t(x) \propto \pone_t(x) \ptwo_t(x)$.  With these choices, the weighted SDE becomes
\begin{align}
    dx_\tau 
    &= \left( -\bref_{1-\tau} + {\sigma_{1-\tau}^2} \nabla \log \pone_{1-\tau} + {\sigma_{1-\tau}^2} \nabla \log \ptwo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} \\
    d\log w_\tau &= \Big( {\langle \nabla, \bref_{1-\tau} \rangle} + \sigma_{1-\tau}^2\langle  \nabla \log \pone_{1-\tau},  \nabla \log \ptwo_{1-\tau} \rangle \Big) d\tau
\end{align}
\end{example}
    \end{mybox}
    \begin{proof} Mostly repeating the above equations, we simplify from \cref{prop:fk_sim}
    \begin{align}
       \begin{split}
    dx_\tau &= \left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} \\ 
    &= \left( -\bref_{1-\tau} + {\sigma_{1-\tau}^2} \nabla \log \pone_{1-\tau} + {\sigma_{1-\tau}^2} \nabla \log \ptwo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} 
      \end{split} \\
    %\begin{split}
d\log w_\tau &= \left(  {\langle \nabla, \bref_{1-\tau} \rangle} +  \frac{\sigma_{1-\tau}^2}{4}\| \nabla \log \pgeo_{1-\tau} \|^2  - \frac{ \sigma_{1-\tau}^2}{4} \| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 \right) d\tau \nonumber \\
&= \Big(   
{\langle \nabla, \bref_{1-\tau} \rangle} + \sigma_{1-\tau}^2\langle  \nabla \log \pone_{1-\tau},  \nabla \log \ptwo_{1-\tau} \rangle \Big) d\tau 
%&=\left( \langle\nabla \log \pgeo_{1-\tau}, \bref_{1-\tau}\rangle +  {\langle \nabla, \bref_{1-\tau} \rangle} +  \frac{\sigma_{1-\tau}^2}{4}\| \nabla \log \pone_{1-\tau} \|^2  + \frac{\sigma_{1-\tau}^2}{4} \| \nabla \log \ptwo_{1-\tau} \|^2 +  \sigma_{1-\tau}^2\langle\nabla \log \pone_{1-\tau}, \nabla \log \ptwo_{1-\tau} \rangle \right) d\tau \nonumber
    %\end{split}
    \end{align}
where in the second line, we simplify using
where in the second line, we simplify using
%\marta{in the second line below should the second and fourth terms contain $p$ and not $q$}\rob{good catch thx}
\begin{align}
&\frac{\sigma_{1-\tau}^2}{4}\| \nabla \log \pone_{1-\tau} + \nabla \log \ptwo_{1-\tau} \|^2  - \frac{ \sigma_{1-\tau}^2}{4} \| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2\nonumber \\
&= \medmath{ \frac{\sigma_{1-\tau}^2}{4} \| \nabla \log \pone_{1-\tau}\|^2 + \frac{\sigma_{1-\tau}^2}{4} \| \nabla \log \ptwo_{1-\tau}\|^2 - \frac{\sigma_{1-\tau}^2}{4} \| \nabla \log \pone_{1-\tau}\|^2 - \frac{\sigma_{1-\tau}^2}{4} \| \nabla \log \ptwo_{1-\tau}\|^2  + 2 \frac{ \sigma_{1-\tau}^2}{2} \langle  \nabla \log \pone_{1-\tau},  \nabla \log \ptwo_{1-\tau} \rangle } \nonumber \\
&=  \sigma_{1-\tau}^2 \langle  \nabla \log \pone_{1-\tau},  \nabla \log \ptwo_{1-\tau} \rangle \nonumber
%\frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pone_{1-\tau}\|^2 + \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \ptwo_{1-\tau}\|^2
\end{align}
\end{proof}

      %\RB{Note, this differs from Kirill's 24-11-14-product-of-FP due to the drift term}

  

%     For the $\gamma=\frac{1}{2}$ geometric average $(\lambda=1)$, we obtain (special case of \cref{ex:clf} below)
%     \begin{align}
%           dx_\tau &= \left( -\bref_{1-\tau} + \frac{\sigma_{1-\tau}^2}{2} \nabla \log \pone_{1-\tau} + \frac{\sigma_{1-\tau}^2}{2} \nabla \log \ptwo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} \\
%           d\log w_\tau &= \left( \frac{\sigma_{1-\tau}^2}{4} \langle\nabla \log \pone_{1-\tau}, \nabla \log \ptwo_{1-\tau} \rangle \right) d\tau
%     \end{align}
% \end{example}
%\marta{eqn 20 -- should $\sigma_\tau$ in front of wiener process be $\sigma_{1-\tau}$?}
\begin{mybox}
\begin{example}[Tempered Distribution]  Consider $\gamma = 1$ and $\lambda = \beta$, leading to the tempered distribution  $\pgeo_t \propto \pone_t^{\beta}$.  Noting that $\gamma(1-\gamma)=0$ and $ \nabla \log \pgeo_{1-\tau} = \beta \nabla \log \pone_{1-\tau} $
\begin{align}
   \begin{split}
dx_\tau &= \left( -\bref_{1-\tau} + \beta \sigma_{1-\tau}^2 \nabla \log \pone_{1-\tau} \right) d\tau + \sigma_{1-\tau} \rev{dW_\tau}  
    \end{split} \\
    \begin{split}
d\log w_\tau 
%&= \left(  (\beta-1) {\langle \nabla, \bref_{1-\tau} \rangle} + \left(1-\frac{1}{\beta}\right) \frac{\sigma_{1-\tau}^2}{2}\| \beta \nabla \log \pone_{1-\tau} \|^2 \right) d\tau  \\
&= \left( (\beta-1) {\langle \nabla, \bref_{1-\tau} \rangle}  + \beta \left(\beta-1\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} \|^2 \right) d\tau
\end{split} 
\end{align}
% \begin{align}
%    \begin{split}
% dx_\tau &= \left( -\bref_{1-\tau} + \beta \sigma_{1-\tau}^2 \nabla \log \pone_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau}  
%     \end{split} \\
%     \begin{split}
% d\log w_\tau &= \left( (\beta-1) {\langle \nabla, \bref_{1-\tau} \rangle} + \left(1-\frac{1}{\beta}\right) \frac{\sigma_{1-\tau}^2}{2}\| \beta \nabla \log \pone_{1-\tau} \|^2 \right) d\tau  \\
% &= \left( (\beta-1) {\langle \nabla, \bref_{1-\tau} \rangle} + \beta \left(\beta-1\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} \|^2 \right) d\tau
% \end{split} 
% \end{align}
%which matches Kirill's derivations in Slack Thurs 11/28.
Note that $\left(1-\frac{1}{\beta}\right) \dfrac{\sigma_{1-\tau}^2}{2}\| \beta \nabla \log \pone_{1-\tau} \|^2  = \beta \left(\beta-1\right) \dfrac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} \|^2 $
\end{example}
\end{mybox}
\begin{mybox}
\begin{example}[Classifier(-Free) Guidance] \label{ex:clf} 
In this case, let $\gamma$ vary freely with $\lambda = 1$, resulting in $\pgeo_t \propto \pone_t^{1-\gamma} \ptwo_t^{\gamma}$ and a drift which is an affine combination of scores
\begin{align}
   \begin{split}
dx_\tau &= \left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} \\
&= \left( -\bref_{1-\tau} + (1-\gamma) \sigma_{1-\tau}^2 \nabla \log \pone_{1-\tau}  + \gamma ~ \sigma_{1-\tau}^2 \nabla \log \ptwo_{1-\tau} \right) d\tau + \sigma_\tau \rev{dW_\tau} 
    \end{split} \\
    \begin{split}
d\log w_\tau &=  
\left( -  \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 \right) d\tau  
%\gamma (1-\gamma) \sigma_{1-\tau}^2\langle\nabla \log \pone_{1-\tau}, \nabla \log \ptwo_{1-\tau} \rangle ~ d\tau \nonumber
\end{split} 
\end{align}
\end{example}
\end{mybox}
For example, $\pone(x)$ may be unconditional and $\ptwo(x|c)$ may be conditional, and the above weighted SDE weights can be used to reweight samples along the trajectory of standard classifier-free guidance sampling (i.e. where both unconditional and conditional scores are learned from denoising score matching with $x_0\sim p_{data}(x)$ and $x_0\sim p_{data}(x|c)$ ).  

%This approach to CFG notably differs from the predictor-corrector interpretation of \citet{bradley2024classifier}, although their discussion may be relevant.  In particular, they show that unadjusted CFG does not sample from $\pone_0^{1-\gamma}\ptwo_0^{\gamma}$ (their Thm 2, intuitively (?) since $\pgeo_{t} = \pone_t^{1-\gamma} \ptwo_t^{\gamma} = \text{noise}_t[ \pone_0]^{1-\gamma}\text{noise}_t[ \ptwo_0]^{\gamma} \neq \text{noise}_t[\pone_0^{1-\gamma}\ptwo_0^{\gamma} ] $ ).  By contrast, our scheme would have guarantees on consistency / asymptotic exactness in the limit of $K \rightarrow \infty$.\footnote{Error or importance weight variance bounds as a function of step-size would also be interesting. } % Of course, more fine-grained bounds in terms of $K$ and discretization steps would be amazing. 
%It would be interesting to characterize the bias of our sampling scheme as a function of discretization steps.
%\end{example}


\subsection{Proof of \cref{prop:fk_sim}}\label{sec:proof}
\begin{proof} consider the target distribution
\begin{align}
\pgeo_{1-\tau}(x) = \frac{1}{\cZ} \pone_{1-\tau}(x)^{\lambda (1-\gamma)} \ptwo_{1-\tau}(x)^{\lambda \gamma}\label{eq:tgt2}
\end{align}
For this target
\begin{align}
\partial_\tau \log \pgeo_{1-\tau} &= 
\lambda (1-\gamma) \partial_\tau \log \pone_{1-\tau} + \lambda \gamma \partial_\tau \log \ptwo_{1-\tau}- \mathbb{E}_{\pgeo_{1-\tau}}[\lambda (1-\gamma)~ \partial_\tau \log \pone_{1-\tau} + \lambda \gamma \partial_\tau \log \ptwo_{1-\tau}]
\end{align}

Recall the form of the Fokker-Planck equation associated with $\pone_{1-\tau}$, for example
\begin{align}
\partial_\tau \pone_{1-\tau} &= - \langle \nabla, \pone_{1-\tau} \left(-\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pone_{1-\tau} \right) \rangle + \frac{\sigma_{1-\tau}^2}{2}\Delta \pone_{1-\tau} \\
\implies \quad \partial_\tau \log \pone_{1-\tau} &=  \langle \nabla \log \pone_{1-\tau},  \bref_{1-\tau} \rangle -  \sigma_{1-\tau}^2 \| \nabla \log \pone_{1-\tau} \|^2 + \langle \nabla, \bref_{1-\tau} \rangle - \sigma_{1-\tau}^2 \Delta \log \pone_{1-\tau} \\
&\qquad \qquad \qquad \qquad  + \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pone_{1-\tau} \|^2 + \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pone_{1-\tau} \nonumber\\
&=\langle \nabla \log \pone_{1-\tau},  \bref_{1-\tau} \rangle  + \langle \nabla, \bref_{1-\tau} \rangle - \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pone_{1-\tau} \|^2 - \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pone_{1-\tau} \label{eq:log_ref}
\end{align}

Using \cref{eq:log_ref} equations for log Fokker-Planck equations, we recognize $\hlb{\nabla \log \pgeo = \lambda (1-\gamma) \nabla \log \pone + \lambda \gamma \nabla \log \ptwo}$ and similarly for $\hlp{\Delta \log \pgeo}$. 


\rob{\textit{We completely ignore $\mathbb{E}[\cdot]$ terms for derivations, and include them in the final result.}... Handle these}


\footnotesize
\begin{align}
    \partial_\tau \log &\pgeo_{1-\tau} = 
\hlb{\lambda (1-\gamma)~ \langle \nabla \log \pone_{1-\tau},  \bref_{1-\tau} \rangle } + \hlo{\lambda (1-\gamma) \langle \nabla, \bref_{1-\tau} \rangle} - \lambda (1-\gamma)~ \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pone_{1-\tau} \|^2  \hlp{-\lambda (1-\gamma)~ \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pone_{1-\tau}} \nonumber \\
&\phantom{\quad}\hlb{+\lambda \gamma \langle \nabla \log \ptwo_{1-\tau},  \bref_{1-\tau} \rangle } +\hlo{\lambda \gamma \langle \nabla, \bref_{1-\tau} \rangle } - \lambda \gamma \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \ptwo_{1-\tau} \|^2 \hlp{- \lambda \gamma \frac{\sigma_{1-\tau}^2}{2} \Delta \log \ptwo_{1-\tau}} \\[1.25ex]
&= \hlb{ \langle \nabla \log \pgeo_{1-\tau} , \bref_{1-\tau} \rangle} + \hlo{\lambda \langle \nabla, \bref_{1-\tau} \rangle} \hlp{- \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pgeo_{1-\tau}} - \lambda (1-\gamma)~ \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pone_{1-\tau} \|^2- \lambda \gamma \frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \ptwo_{1-\tau} \|^2 \label{eq:last_terms}
\end{align}
\normalsize
\begin{lemma} The following identity holds
    \begin{align}
        {-\lambda(1-\gamma)\|\nabla \log \pone \|^2 -\lambda \gamma \|\nabla \log \ptwo\|^2 = - \lambda \gamma (1-\gamma) \| \nabla \log \pone - \nabla \log \ptwo \|^2 - \frac{1}{\lambda} \| \lambda(1-\gamma) \nabla \log \pone + \lambda \gamma \nabla \log \ptwo \|^2  } \label{eq:sub}
    \end{align}
\end{lemma}
\begin{proof}
    

 \textit{Lemma: (Building up to \cref{eq:sub})}  Our goal is to substitute the last two terms in \cref{eq:last_terms} with something involving $\|\lambda (1-\gamma)\nabla \log \pone + \lambda\gamma \nabla \log \ptwo\|^2 = \| \nabla \log \pgeo \|^2$, which we can then combine with the Laplacian $\Delta \log \pgeo$ to obtain a term of $\Delta \pgeo$.  Expanding $\| \nabla \log \pgeo \|^2$ , we have
 %To handle the last two terms consider $\gamma = \gamma^2 +  \gamma (1-\gamma)$ as above. 
%\small
\begin{align*}
\| \nabla \log \pgeo \|^2 &= \|\lambda (1-\gamma)\nabla \log \pone + \lambda \gamma \nabla \log \ptwo\|^2 \\
&=
\lambda^2 (1-\gamma)^2 \|\nabla \log \pone\|^2 + \lambda^2 \gamma^2 \|\nabla \log \ptwo \|^2 + 2 \lambda^2 \gamma (1-\gamma) \langle\nabla \log \pone, \nabla \log \ptwo \rangle
%\implies -\lambda&\left( \hlb{\lambda (1-\gamma) \|\nabla \log \pone\|^2 + \lambda \gamma \|\nabla \log \ptwo \|^2 }\right) =  2 \lambda^2 \gamma (1-\gamma) \langle\nabla \log \pone, \nabla \log \ptwo \rangle - \| \nabla \log \pgeo \|^2
\end{align*}
\normalsize
Next, we use the fact that  $(1-\gamma)^2u = (1-\gamma) u- \gamma(1-\gamma) u$ and, similarly, $ \gamma^2 u = \gamma  u  - \gamma (1-\gamma) u$, to recognize terms with similar coefficients to \cref{eq:last_terms},
%(similarly for $\gamma \gets 1-\gamma$, namely
\begin{align}
   \| \nabla \log \pgeo \|^2 &=  \lambda^2 (1-\gamma) \|\nabla \log \pone\|^2- \lambda^2 \gamma (1-\gamma) \|\nabla \log \pone\|^2   + 2 \lambda^2 \gamma (1-\gamma) \langle\nabla \log \pone, \nabla \log \ptwo \rangle \nonumber \\
   &\phantom{==} + \lambda^2 \gamma \|\nabla \log \ptwo \|^2 - \lambda^2 \gamma (1-\gamma) \|\nabla \log \ptwo \|^2  \nonumber 
\end{align}
Rearranging and dividing by $\lambda$
\begin{align}
     &-\lambda (1-\gamma) \|\nabla \log \pone \|^2 -\lambda \gamma \|\nabla \log \ptwo\|^2 \nonumber \\
     &= -\lambda \gamma (1-\gamma) \|\nabla \log \pone \|^2 - \lambda \gamma (1-\gamma) \|\nabla \log \ptwo \|^2 + 2 \lambda \gamma (1-\gamma) \langle\nabla \log \pone, \nabla \log \ptwo \rangle  -\frac{1}{\lambda} \| \nabla \log \pgeo \|^2 \nonumber \\
     &= - \lambda \gamma (1-\gamma) \| \nabla \log \pone - \nabla \log \ptwo \|^2 - \frac{1}{\lambda} \| \nabla \log \pgeo \|^2  \nonumber \\
     &\implies \medmath{-\lambda(1-\gamma)\|\nabla \log \pone \|^2 -\lambda \gamma \|\nabla \log \ptwo\|^2 = - \lambda \gamma (1-\gamma) \| \nabla \log \pone - \nabla \log \ptwo \|^2 - \frac{1}{\lambda} \| \lambda(1-\gamma) \nabla \log \pone + \lambda \gamma \nabla \log \ptwo \|^2  }  \nonumber
\end{align}
which is the desired identity.
%
\end{proof}


\textit{Completing the Weighted SDE Proof} 
Substituting \cref{eq:sub} into \cref{eq:last_terms} above (noting that we multiply by $\dfrac{\sigma_{1-\tau}^2}{2}$)
\small
\begin{align}
   \partial_\tau \log \pgeo_{1-\tau} &= { \langle \nabla \log \pgeo , \bref_{1-\tau} \rangle} + \lambda {\langle \nabla, \bref_{1-\tau} \rangle} {- \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pgeo_{1-\tau}}  - \frac{1}{\lambda}\frac{\sigma_{1-\tau}^2}{2} \| \nabla \log \pgeo_{1-\tau} \|^2  \\
   &\phantom{=} \qquad \qquad\qquad\qquad \qquad \qquad  \hfill  - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 \nonumber \\
   &=  \langle \nabla \log \pgeo_{1-\tau} , \bref_{1-\tau} \rangle + \langle \nabla, \bref_{1-\tau} \rangle  +  (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} \hlp{- \frac{\sigma_{1-\tau}^2}{2} \Delta \log \pgeo_{1-\tau} - \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2}  \\
   &\phantom{======}+ \left(\hlp{1}-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2 
   - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 \nonumber \\
   &= \hlb{\frac{-1}{\pgeo_{1-\tau}} \left\langle \nabla,\pgeo_{1-\tau}\left( -\bref_{1-\tau}  \right) \right\rangle } - \hlp{\frac{1}{\pgeo_{1-\tau}} \frac{\sigma_{1-\tau}^2}{2} \Delta \pgeo_{1-\tau}} \\
   &\phantom{======}~  + (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} +
\left(\hlp{1}-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2 
   - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2 \nonumber 
\end{align}
\normalsize
Finally, let's multiply both sides by $\pgeo_{1-\tau}$ to obtain an expression for $\partial_\tau \pgeo_{1-\tau}$.   We also move $\Delta \pgeo_{1-\tau}$ inside the drift to simulate the correct direction,
\begin{align}
   \partial_\tau  \pgeo_{1-\tau}  &= -\left\langle \nabla,\pgeo_{1-\tau}\left( -\bref_{1-\tau} + \sigma_{1-\tau}^2 \nabla \log \pgeo_{1-\tau} \right) \right\rangle + \frac{\sigma_{1-\tau}^2}{2} \Delta \pgeo_{1-\tau} \\
   &\phantom{=} + \pgeo_{1-\tau}\Bigg(   (\lambda-1) {\langle \nabla, \bref_{1-\tau} \rangle} +
\left(\hlp{1}-\frac{1}{\lambda}\right) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pgeo_{1-\tau} \|^2 \nonumber \\
 &\phantom{= + \pgeo_{1-\tau}\Bigg(}
 - \lambda \gamma (1-\gamma) \frac{\sigma_{1-\tau}^2}{2}\| \nabla \log \pone_{1-\tau} - \nabla \log \ptwo_{1-\tau} \|^2  \Bigg)
   \nonumber 
\end{align}
\normalsize
% Recognizing the square in the latter terms and rearranging to isolate the term appearing above, we have
% \small
% \begin{align}
% \lambda (1-\gamma) \|\nabla \log \pone\|^2 + \lambda \gamma \|\nabla \log \ptwo \|^2 = \lambda \gamma (1-\gamma)\|\nabla \log \pone - \nabla \log \ptwo \|^2 + \|\lambda (1-\gamma)\nabla \log \pone + \lambda \gamma \nabla \log \ptwo\|^2
% \end{align}
% \normalsize
% where we recognize $\|\lambda (1-\gamma)\nabla \log \pone + \gamma \nabla \log \ptwo\|^2 = \| \nabla \log \pgeo \|^2$
\end{proof}

==> old_derivations/old_tables.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        % \vspace*{-.25cm}
        \captionof{table}{LJ-13 sampling task with various SDEs, with performance measured by mean $\pm$ standard deviation over 3 seeds. The starting temperature is $T_L=2$, annealed to target temperatures $T_S=0.8$ and $T_S=1.5$. The DEM samples are generated with a model trained at those corresponding target temperatures.} 
        \vspace*{.1cm}
        \resizebox{\linewidth}{!}{%
        \begin{tabular}{llcccc}
        \toprule
        Target Temp. & SDE Type & FKC & Distance-$\mathcal{W}_2$ & Energy-$\mathcal{W}_1$ & Energy-$\mathcal{W}_2$ \\
        \midrule
        \multirow[t]{6}{*}{\makecell[c]{ \\ \\ \\ \\ 0.8 \\ $(\beta=2.5$)}} 
            & \multirow{2}{*}{Target Score} & \no & \textbf{0.912 $\pm$ 0.016} & 14.521 $\pm$ 0.085 & 14.602 $\pm$ 0.076 \\
            &  & \yes & 0.928 $\pm$ 0.009 & \textbf{5.513 $\pm$ 0.586} & \textbf{5.591 $\pm$ 0.563} \\
        \arrayrulecolor{gray}\cline{2-6}
            & \multirow{2}{*}{Tempered Noise} & \no & 0.924 $\pm$ 0.001 & 6.206 $\pm$ 0.007 & 6.272 $\pm$ 0.017 \\
            &  & \yes & 0.930 $\pm$ 0.020 & 6.438 $\pm$ 0.994 & 6.620 $\pm$ 0.998 \\
            0.082 $\pm$ 0.007 & 6.487 $\pm$ 0.056 & 8.501 $\pm$ 0.283 \\
            
        \arrayrulecolor{gray}\cline{2-6}
            & DEM & --- & 0.010 $\pm$ 0.001 & 9.910 $\pm$ 0.004 & 9.921 $\pm$ 0.004  \\
        \arrayrulecolor{black} \midrule
        \multirow[t]{6}{*}{\makecell[c]{ \\ \\ \\ \\ 1.5 \\ $(\beta=1.33$)}} 
            & \multirow{2}{*}{Target Score} & \no & 0.222 $\pm$ 0.011 & 5.152 $\pm$ 0.040 & 5.211 $\pm$ 0.049 \\
            &  & \yes & 0.225 $\pm$ 0.009 & 3.249 $\pm$ 0.003 & 3.269 $\pm$ 0.004\\
        \arrayrulecolor{gray}\cline{2-6}
            & \multirow{2}{*}{Tempered Noise} & \no & \textbf{0.215 $\pm$ 0.004} & 2.075 $\pm$ 0.010 & 2.236 $\pm$ 0.005 \\
            &  & \yes & 0.217 $\pm$ 0.009 & \textbf{0.703 $\pm$ 0.017} & \textbf{0.888 $\pm$ 0.048} \\
        \arrayrulecolor{gray}\cline{2-6} 
            & DEM & --- & 0.074 $\pm$ 0.001 & 4.461 $\pm$ 0.024 & 5.144 $\pm$ 0.042 \\
        \arrayrulecolor{black}\bottomrule
        \end{tabular}%
        }
        \label{tab:lj_results}
    \end{minipage} \hfill
       \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=.7\linewidth]{pics/LJ_energy_w2_vs_temp.png}
        \vspace*{-.4cm}
        \caption{2-Wasserstein between energy distributions of MCMC samples from the annealed target distribution and our methods at different temperatures. Note the training temperature $\ltemp=2$.}
        \label{fig:LJ_energy_W2}
    \end{minipage}%
    \vspace{-2mm}
\end{figure*}

==> tables/3dligand_twoproteins_14pairs.tex <==
\begin{table*}[t]
\centering
\vspace{-0.9em}
\caption{Docking scores of generated ligands for 14 protein target pairs (\texttt{P$_1$}, \texttt{P$_2$}). We generate 32 ligands for 5 molecule lengths for each protein pair using the Target Score SDE. Lower docking scores are better. Values are reported as averages over all generated molecules in each run, except for top-1. "Better than ref." is the percentage of ligands with better docking scores than known reference molecules for \textit{both} targets (the mean docking score for the reference molecules is $-8.255_{\pm 1.849}$). We also report the diversity, validity \& uniqueness, and quality. $^1$TargetDiff from ~\citet{guan20233d}, $^2$DualDiff from ~\citet{zhou2024reprogramming}.} 
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule

  & 
 & (\texttt{P$_1$} * \texttt{P$_2$}) ($\uparrow$) & max(\texttt{P$_1$}, \texttt{P$_2$}) ($\downarrow$) & \texttt{P$_1$} ($\downarrow$) & \texttt{P$_2$} ($\downarrow$) & \texttt{P$_1$} top-1 ($\downarrow$) & \texttt{P$_2$} top-1 ($\downarrow$) & Better than ref. ($\uparrow$) & Div. ($\uparrow$) & Val. \& Uniq. ($\uparrow$) & Qual. ($\uparrow$) \\
 \midrule

% \multicolumn{2}{l}{Reference} & --- & --- & --- & --- & $-8.255_{\pm 1.849}$ & $-8.255_{\pm 1.849}$ & --- & $0.920$ & $0.200$ & $0.086$\\

 
  \multicolumn{2}{l}{\texttt{P$_1$} only$^1$} & $62.770_{\pm 23.741}$ & $-7.301_{\pm 1.902}$ & $-8.384_{\pm 1.513}$ & $-7.441_{\pm 1.934}$ & $\mathbf{-12.717_{\pm 1.846}}$ & $-10.822_{\pm 0.996}$ & $0.321_{\pm 0.365}$ & $\mathbf{0.889_{\pm 0.011}}$ & $0.946_{\pm 0.067}$ & $0.161_{\pm 0.160}$ \\
 \midrule
 \midrule
 
 $\beta$ & FKC
 & (\texttt{P$_1$} * \texttt{P$_2$}) ($\uparrow$) & max(\texttt{P$_1$}, \texttt{P$_2$}) ($\downarrow$) & \texttt{P$_1$} ($\downarrow$) & \texttt{P$_2$} ($\downarrow$) & \texttt{P$_1$} top-1 ($\downarrow$) & \texttt{P$_2$} top-1 ($\downarrow$) & Better than ref. ($\uparrow$) & Div. ($\uparrow$) & Val. \& Uniq. ($\uparrow$) & Qual. ($\uparrow$) \\ 
 \midrule

\multirow[c]{2}{*}{0.5} & \no$^2$ & $64.345_{\pm 21.535}$ & $-7.141_{\pm 2.117}$ & $-7.903_{\pm 1.994}$ & $-7.960_{\pm 1.665}$ & $-10.749_{\pm 1.310}$ & $-11.032_{\pm 1.311}$ & $0.247_{\pm 0.339}$ & $0.886_{\pm 0.008}$ & $0.890_{\pm 0.211}$ & $0.236_{\pm 0.202}$ \\

 & \yes$\,\,$ & $64.056_{\pm 31.212}$ & $-6.858_{\pm 3.259}$ & $-7.892_{\pm 2.902}$ & $-7.923_{\pm 2.419}$ & $-11.222_{\pm 1.589}$ & $-10.978_{\pm 1.667}$ & $0.282_{\pm 0.371}$ & $0.877_{\pm 0.015}$ & $\mathbf{0.947_{\pm 0.106}}$ & $0.198_{\pm 0.185}$\\
 
\midrule

\multirow[c]{2}{*}{1.0} & \no$\,\,$ & $69.031_{\pm 21.614}$ & $-7.541_{\pm 1.738}$ & $-8.235_{\pm 1.712}$ & $-8.298_{\pm 1.531}$ & $-11.165_{\pm 1.484}$ & $-11.096_{\pm 1.195}$ & $0.285_{\pm 0.361}$ & $0.886_{\pm 0.009}$ & $0.898_{\pm 0.186}$ & $0.239_{\pm 0.199}$ \\

 & \yes$\,\,$ & $69.829_{\pm 32.702}$ & $-7.399_{\pm 2.932}$ & $-8.514_{\pm 1.816}$ & $-8.271_{\pm 2.877}$ & $-11.317_{\pm 1.432}$ & $\mathbf{-11.190_{\pm 1.005}}$ & $0.327_{\pm 0.392}$ & $0.847_{\pm 0.023}$ & $0.922_{\pm 0.098}$ & $0.223_{\pm 0.210}$ \\
\midrule

\multirow[c]{2}{*}{2.0} & \no$\,\,$ &  
$68.115_{\pm 18.557}$ & $-7.396_{\pm 2.025}$ & $-8.211_{\pm 1.663}$ & $-8.113_{\pm 1.617}$ & $-11.303_{\pm 1.080}$ & $-10.776_{\pm 1.088}$ & $0.279_{\pm 0.358}$ & $0.882_{\pm 0.014}$ & $0.944_{\pm 0.160}$ & $\mathbf{0.271_{\pm 0.216}}$ \\


 & \yes$\,\,$ & $\mathbf{75.535_{\pm 23.261}}$ & $\mathbf{-7.913_{\pm 1.619}}$ & $\mathbf{-8.601_{\pm 1.623}}$ & $\mathbf{-8.664_{\pm 1.552}}$ & $-11.406_{\pm 1.361}$ & $-11.128_{\pm 1.305}$ & $\mathbf{0.341_{\pm 0.429}}$ & $0.808_{\pm 0.047}$ & $0.876_{\pm 0.091}$ & $0.234_{\pm 0.232}$ \\


\bottomrule
\end{tabular}
}
\label{tab:dualtarget_best}
\end{table*}

==> tables/3dligand_twoproteins_ablation_2.tex <==
\begin{table*}[t]
\centering

\vspace{-0.9em}
\caption{sdfskjdhfs}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule

 SDE Type & $\beta$ & FKC & $t_{\text{max}}$ & (\texttt{P$_1$} * \texttt{P$_2$}) ($\uparrow$) & max(\texttt{P$_1$}, \texttt{P$_2$}) ($\downarrow$) & \texttt{P$_1$} ($\downarrow$) & \texttt{P$_2$} ($\downarrow$) & \texttt{P$_1$} top-1 ($\downarrow$) & \texttt{P$_2$} top-1 ($\downarrow$) & Better than ref. ($\uparrow$) & Div. ($\uparrow$) & Val. \& Uniq. ($\uparrow$) & Qual. ($\uparrow$) \\ \midrule

 \cellcolor{highlightturq} Target Score &  \multirow[c]{4}{*}{0.5} & \no & --- & $67.657_{\pm 11.985}$ & $-7.667_{\pm 0.687}$ & $-8.377_{\pm 0.661}$ & $-7.986_{\pm 0.948}$ & $-11.718_{\pm 0.000}$ & $-10.450_{\pm 0.000}$ & $0.251_{\pm 0.199}$ & $0.886_{\pm 0.006}$ & $0.969_{\pm 0.062}$ & $0.244_{\pm 0.161}$ \\

  \cellcolor{highlightpurple} Target Score &   & \yes & 0.6 & $77.100_{\pm 16.533}$ & $-8.243_{\pm 0.949}$ & $-9.112_{\pm 0.898}$ & $-8.337_{\pm 1.045}$ & $-12.191_{\pm 0.000}$ & $-10.833_{\pm 0.000}$ & $0.417_{\pm 0.337}$ & $0.877_{\pm 0.008}$ & $0.975_{\pm 0.023}$ & $0.212_{\pm 0.155}$ \\

 \cellcolor{highlightorange}  Tempered Noise &  & \no & --- & $71.606_{\pm 15.139}$ & $-7.838_{\pm 0.872}$ & $-8.727_{\pm 0.878}$ & $-8.085_{\pm 1.088}$ & $-12.382_{\pm 0.000}$ & $-11.038_{\pm 0.000}$ & $0.362_{\pm 0.274}$ & $0.887_{\pm 0.007}$ & $0.944_{\pm 0.098}$ & $0.300_{\pm 0.212}$ \\

 \cellcolor{lightgray} Tempered Noise &  & \yes & 0.6 & $78.501_{\pm 15.383}$ & $-8.323_{\pm 0.919}$ & $-9.127_{\pm 0.770}$ & $-8.496_{\pm 1.100}$ & $-11.251_{\pm 0.000}$ & $-10.976_{\pm 0.000}$ & $0.496_{\pm 0.308}$ & $0.879_{\pm 0.016}$ & $0.931_{\pm 0.064}$ & $0.250_{\pm 0.163}$ \\
 
\midrule

 --- & 1.0 & \no & --- & $73.366_{\pm 14.423}$ & $-7.929_{\pm 0.763}$ & $-8.843_{\pm 0.899}$ & $-8.174_{\pm 0.989}$ & $-11.807_{\pm 0.000}$ & $-11.671_{\pm 0.000}$ & $0.378_{\pm 0.311}$ & $0.884_{\pm 0.008}$ & $0.962_{\pm 0.023}$ & $0.231_{\pm 0.170}$ \\

  --- & 1.0 & \yes & 0.6 & $80.077_{\pm 14.422}$ & $-8.355_{\pm 0.805}$ & $-9.154_{\pm 0.617}$ & $-8.681_{\pm 1.150}$ & $-12.194_{\pm 0.000}$ & $-11.267_{\pm 0.000}$ & $0.406_{\pm 0.304}$ & $0.842_{\pm 0.027}$ & $0.919_{\pm 0.096}$ & $0.238_{\pm 0.184}$ \\
  
\midrule

Target Score & \multirow[c]{6}{*}{1.5} & \no & --- &  $75.213_{\pm 15.779}$ & $-8.085_{\pm 0.856}$ & $-8.980_{\pm 0.935}$ & $-8.258_{\pm 1.024}$ & $-12.162_{\pm 0.000}$ & $-10.951_{\pm 0.000}$ & $0.402_{\pm 0.339}$ & $0.880_{\pm 0.012}$ & $0.988_{\pm 0.015}$ & $0.250_{\pm 0.159}$ \\

Target Score & & \yes & 0.4 &  $74.558_{\pm 14.361}$ & $-7.961_{\pm 0.785}$ & $-8.883_{\pm 0.885}$ & $-8.322_{\pm 1.083}$ & $-11.450_{\pm 0.000}$ & $-11.411_{\pm 0.000}$ & $0.372_{\pm 0.328}$ & $0.883_{\pm 0.021}$ & $0.981_{\pm 0.038}$ & $0.262_{\pm 0.222}$ \\

Target Score & & \yes & 0.5 &  $80.421_{\pm 16.567}$ & $-8.365_{\pm 0.905}$ & $-9.314_{\pm 0.882}$ & $-8.539_{\pm 1.077}$ & $-12.207_{\pm 0.000}$ & $-10.339_{\pm 0.000}$ & $0.494_{\pm 0.378}$ & $0.867_{\pm 0.014}$ & $0.994_{\pm 0.012}$ & $0.288_{\pm 0.233}$ \\


 Target Score & & \yes & 0.6 &  $83.405_{\pm 19.024}$ & $-8.530_{\pm 1.070}$ & $-9.516_{\pm 1.083}$ & $-8.646_{\pm 1.098}$ & $-11.585_{\pm 0.000}$ & $-10.544_{\pm 0.000}$ & $0.485_{\pm 0.441}$ & $0.820_{\pm 0.024}$ & $0.925_{\pm 0.078}$ & $0.244_{\pm 0.196}$ \\

 Target Score & & \yes & 0.7 &   $83.100_{\pm 19.354}$ & $-8.434_{\pm 0.912}$ & $-9.420_{\pm 1.229}$ & $-8.723_{\pm 1.227}$ & $-12.101_{\pm 0.000}$ & $-10.402_{\pm 0.000}$ & $0.503_{\pm 0.441}$ & $0.799_{\pm 0.030}$ & $0.888_{\pm 0.094}$ & $0.162_{\pm 0.205}$ \\

 Target Score & & \yes & 1.0 &   $75.798_{\pm 32.984}$ & $-7.438_{\pm 2.507}$ & $-8.582_{\pm 3.200}$ & $-8.829_{\pm 1.193}$ & $-12.724_{\pm 0.000}$ & $-10.227_{\pm 0.000}$ & $0.446_{\pm 0.454}$ & $0.651_{\pm 0.102}$ & $0.475_{\pm 0.169}$ & $0.100_{\pm 0.157}$ \\

\midrule

Target Score & \multirow[c]{8}{*}{2.0} & \no & --- &  $75.551_{\pm 16.345}$ & $-8.089_{\pm 0.899}$ & $-8.966_{\pm 0.884}$ & $-8.309_{\pm 1.112}$ & $-12.320_{\pm 0.000}$ & $-10.118_{\pm 0.000}$ & $0.391_{\pm 0.331}$ & $0.881_{\pm 0.011}$ & $0.994_{\pm 0.012}$ & $0.288_{\pm 0.179}$ \\

Tempered Noise & & \no & --- &  $75.868_{\pm 16.154}$ & $-8.045_{\pm 0.909}$ & $-8.977_{\pm 0.978}$ & $-8.352_{\pm 1.095}$ & $-11.909_{\pm 0.000}$ & $-10.803_{\pm 0.000}$ & $0.460_{\pm 0.390}$ & $0.874_{\pm 0.008}$ & $0.994_{\pm 0.012}$ & $0.262_{\pm 0.186}$ \\

Target Score &  & \yes & 0.4 &  $79.734_{\pm 17.631}$ & $-8.331_{\pm 0.981}$ & $-9.283_{\pm 0.968}$ & $-8.467_{\pm 1.133}$ & $-11.547_{\pm 0.000}$ & $-11.286_{\pm 0.000}$ & $0.498_{\pm 0.388}$ & $0.876_{\pm 0.012}$ & $0.988_{\pm 0.015}$ & $0.306_{\pm 0.234}$ \\

Target Score &  & \yes & 0.5 &  $84.949_{\pm 19.056}$ & $-8.569_{\pm 0.978}$ & $-9.529_{\pm 1.018}$ & $-8.796_{\pm 1.220}$ & $-12.795_{\pm 0.000}$ & $-11.069_{\pm 0.000}$ & $0.514_{\pm 0.423}$ & $0.851_{\pm 0.025}$ & $0.938_{\pm 0.059}$ & $0.244_{\pm 0.160}$ \\

Target Score &  & \yes & 0.6 &  $87.983_{\pm 22.856}$ & $-8.790_{\pm 1.231}$ & $-9.619_{\pm 1.101}$ & $-8.988_{\pm 1.442}$ & $-13.314_{\pm 0.000}$ & $-11.457_{\pm 0.000}$ & $0.569_{\pm 0.468}$ & $0.818_{\pm 0.011}$ & $0.888_{\pm 0.073}$ & $0.212_{\pm 0.223}$ \\

Tempered Noise &  & \yes & 0.6 &  $79.696_{\pm 18.087}$ & $-8.229_{\pm 0.997}$ & $-9.104_{\pm 0.921}$ & $-8.681_{\pm 1.481}$ & $-11.456_{\pm 0.000}$ & $-10.998_{\pm 0.000}$ & $0.464_{\pm 0.429}$ & $0.796_{\pm 0.038}$ & $0.838_{\pm 0.109}$ & $0.331_{\pm 0.274}$ \\

Target Score &  & \yes & 0.7 &  $85.168_{\pm 21.258}$ & $-8.574_{\pm 1.097}$ & $-9.514_{\pm 1.028}$ & $-8.827_{\pm 1.452}$ & $-13.168_{\pm 0.000}$ & $-10.366_{\pm 0.000}$ & $0.593_{\pm 0.484}$ & $0.786_{\pm 0.034}$ & $0.806_{\pm 0.096}$ & $0.231_{\pm 0.224}$ \\

Tempered Noise &  & \yes & 0.7 &  $84.969_{\pm 18.906}$ & $-8.531_{\pm 0.980}$ & $-9.809_{\pm 1.170}$ & $-8.545_{\pm 0.991}$ & $-12.597_{\pm 0.000}$ & $-10.659_{\pm 0.000}$ & $0.589_{\pm 0.427}$ & $0.796_{\pm 0.035}$ & $0.850_{\pm 0.121}$ & $0.262_{\pm 0.154}$ \\

\bottomrule
\end{tabular}
}
\label{tab:dualtarget_ablation}
\end{table*}

==> tables/3dligand_twoproteins_ablation_rebuttal.tex <==
\begin{table*}[t]
\centering

\vspace{-0.9em}
\caption{Performance of generated molecules with different SDE settings. We generate 32 molecules for 5 molecule sizes for one protein pair for each setting. Lower docking scores are better. Values are reported as averages over all generated molecules in each run. "Better than ref." is the percentage of ligands with better docking scores than known reference molecules for \textit{both} targets (the mean docking score for the reference molecules is $-8.255_{\pm 1.849}$). We also report the diversity, validity \& uniqueness, and quality, which refers to the percentage of molecules that are valid, unique, have QED $\geq 0.6$ and SA $\leq 4.0$~\citep{lee2025genmol}. Bolded values are the best metrics within each set of midlines. For {\small$\beta = 1$}, target score and tempering noise are equivalent.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule

  $\beta$ & FKC & $t_{\text{max}}$ & SDE Type & (\texttt{P$_1$} * \texttt{P$_2$}) ($\uparrow$) & max(\texttt{P$_1$}, \texttt{P$_2$}) ($\downarrow$) & \texttt{P$_1$} ($\downarrow$) & \texttt{P$_2$} ($\downarrow$) & Better than ref. ($\uparrow$) & Div. ($\uparrow$) & Val. \& Uniq. ($\uparrow$) & Qual. ($\uparrow$) \\ \midrule
  
     \cellcolor{highlightturq} $0.5$ &  \no & --- & Target Score & $67.657_{\pm 11.985}$ & $-7.667_{\pm 0.687}$ & $-8.377_{\pm 0.661}$ & $-7.986_{\pm 0.948}$ & $0.251_{\pm 0.199}$ & $\mathbf{0.886_{\pm 0.006}}$ & $0.969_{\pm 0.062}$ & $0.244_{\pm 0.161}$ \\

     \cellcolor{highlightturq} $1.0$ &   \no & --- & Target Score & $73.366_{\pm 14.423}$ & $-7.929_{\pm 0.763}$ & $-8.843_{\pm 0.899}$ & $-8.174_{\pm 0.989}$ & $0.378_{\pm 0.311}$ & $0.884_{\pm 0.008}$ & $0.962_{\pm 0.023}$ & $0.231_{\pm 0.170}$ \\

     \cellcolor{highlightturq} $1.5$  & \no & --- &  Target Score & $75.213_{\pm 15.779}$ & $-8.085_{\pm 0.856}$ & $-8.980_{\pm 0.935}$ & $-8.258_{\pm 1.024}$ & $\mathbf{0.402_{\pm 0.339}}$ & $0.880_{\pm 0.012}$ & $0.988_{\pm 0.015}$ & $0.250_{\pm 0.159}$ \\

     \cellcolor{highlightturq} $2.0$  & \no & --- &  Target Score & $\mathbf{75.551_{\pm 16.345}}$ & $\mathbf{-8.089_{\pm 0.899}}$ & $\mathbf{-8.966_{\pm 0.884}}$ & $\mathbf{-8.309_{\pm 1.112}}$ & $0.391_{\pm 0.331}$ & $0.881_{\pm 0.011}$ & $\mathbf{0.994_{\pm 0.012}}$ & $\mathbf{0.288_{\pm 0.179}}$ \\

     \midrule

$1.5$ &   \cellcolor{highlightgray} \no & --- & Target Score & $75.213_{\pm 15.779}$ & $\mathbf{-8.085_{\pm 0.856}}$ & $\mathbf{-8.980_{\pm 0.935}}$ & $-8.258_{\pm 1.024}$ & $0.402_{\pm 0.339}$ & $\mathbf{0.880_{\pm 0.012}}$ & $\mathbf{0.988_{\pm 0.015}}$ & $\mathbf{0.250_{\pm 0.159}}$ \\ 

$1.5$ &   \cellcolor{highlightgray} \yes & --- & Target Score & $\mathbf{75.798_{\pm 32.984}}$ & $-7.438_{\pm 2.507}$ & $-8.582_{\pm 3.200}$ & $\mathbf{-8.829_{\pm 1.193}}$ & $\mathbf{0.446_{\pm 0.454}}$ & $0.651_{\pm 0.102}$ & $0.475_{\pm 0.169}$ & $0.100_{\pm 0.157}$ \\ 

     \midrule

$2.0$ &   \cellcolor{highlightgray} \no & --- & Target Score & $75.551_{\pm 16.345}$ & $-8.089_{\pm 0.899}$ & $-8.966_{\pm 0.884}$ & $-8.309_{\pm 1.112}$ & $0.391_{\pm 0.331}$ & $\mathbf{0.881_{\pm 0.011}}$ & $\mathbf{0.994_{\pm 0.012}}$ & $\mathbf{0.288_{\pm 0.179}}$ \\ 

$2.0$ &   \cellcolor{highlightgray} \yes & --- & Target Score & $\mathbf{91.845_{\pm 28.421}}$ & $\mathbf{-8.977_{\pm 1.433}}$ & $\mathbf{-9.984_{\pm 1.533}}$ & $\mathbf{-8.978_{\pm 1.434}}$ & $\mathbf{0.671_{\pm 0.419}}$ & $0.617_{\pm 0.049}$ & $0.475_{\pm 0.132}$ & $0.044_{\pm 0.073}$ \\ 

     \midrule


$1.5$ &  \yes & \cellcolor{highlightpurple} 0.4 & Target Score & $74.558_{\pm 14.361}$ & $-7.961_{\pm 0.785}$ & $-8.883_{\pm 0.885}$ & $-8.322_{\pm 1.083}$ & $0.372_{\pm 0.328}$ & $\mathbf{0.883_{\pm 0.021}}$ & $0.981_{\pm 0.038}$ & $0.262_{\pm 0.222}$ \\ 

$1.5$ &  \yes & \cellcolor{highlightpurple} 0.5 & Target Score & $80.421_{\pm 16.567}$ & $-8.365_{\pm 0.905}$ & $-9.314_{\pm 0.882}$ & $-8.539_{\pm 1.077}$ & $0.494_{\pm 0.378}$ & $0.867_{\pm 0.014}$ & $\mathbf{0.994_{\pm 0.012}}$ & $\mathbf{0.288_{\pm 0.233}}$ \\ 

$1.5$ &  \yes & \cellcolor{highlightpurple} $0.6$ & Target Score &  $\mathbf{83.405_{\pm 19.024}}$ & $\mathbf{-8.530_{\pm 1.070}}$ & $\mathbf{-9.516_{\pm 1.083}}$ & $-8.646_{\pm 1.098}$ & $0.485_{\pm 0.441}$ & $0.820_{\pm 0.024}$ & $0.925_{\pm 0.078}$ & $0.244_{\pm 0.196}$ \\


$1.5$ &  \yes & \cellcolor{highlightpurple} $0.7$ & Target Score & $83.100_{\pm 19.354}$ & $-8.434_{\pm 0.912}$ & $-9.420_{\pm 1.229}$ & $-8.723_{\pm 1.227}$ & $\mathbf{0.503_{\pm 0.441}}$ & $0.799_{\pm 0.030}$ & $0.888_{\pm 0.094}$ & $0.162_{\pm 0.205}$ \\


$1.5$ &  \yes & \cellcolor{highlightpurple} $1.0$ & Target Score & $75.798_{\pm 32.984}$ & $-7.438_{\pm 2.507}$ & $-8.582_{\pm 3.200}$ & $\mathbf{-8.829_{\pm 1.193}}$ & $0.446_{\pm 0.454}$ & $0.651_{\pm 0.102}$ & $0.475_{\pm 0.169}$ & $0.100_{\pm 0.157}$ \\

\midrule

$2.0$ &  \yes & \cellcolor{highlightpurple} 0.4 & Target Score & $79.734_{\pm 17.631}$ & $-8.331_{\pm 0.981}$ & $-9.283_{\pm 0.968}$ & $-8.467_{\pm 1.133}$ & $0.498_{\pm 0.388}$ & $\mathbf{0.876_{\pm 0.012}}$ & $\mathbf{0.988_{\pm 0.015}}$ & $\mathbf{0.306_{\pm 0.234}}$ \\ 


$2.0$ &  \yes & \cellcolor{highlightpurple} 0.5 & Target Score & $84.949_{\pm 19.056}$ & $-8.569_{\pm 0.978}$ & $-9.529_{\pm 1.018}$ & $-8.796_{\pm 1.220}$ & $0.514_{\pm 0.423}$ & $0.851_{\pm 0.025}$ & $0.938_{\pm 0.059}$ & $0.244_{\pm 0.160}$ \\ 

$2.0$ &  \yes & \cellcolor{highlightpurple} 0.6 & Target Score & $87.983_{\pm 22.856}$ & $-8.790_{\pm 1.231}$ & $-9.619_{\pm 1.101}$ & $\mathbf{-8.988_{\pm 1.442}}$ & $0.569_{\pm 0.468}$ & $0.818_{\pm 0.011}$ & $0.888_{\pm 0.073}$ & $0.212_{\pm 0.223}$ \\ 

$2.0$ &  \yes & \cellcolor{highlightpurple} 0.7 & Target Score & $85.168_{\pm 21.258}$ & $-8.574_{\pm 1.097}$ & $-9.514_{\pm 1.028}$ & $-8.827_{\pm 1.452}$ & $0.593_{\pm 0.484}$ & $0.786_{\pm 0.034}$ & $0.806_{\pm 0.096}$ & $0.231_{\pm 0.224}$ \\ 

$2.0$ &  \yes & \cellcolor{highlightpurple} 1.0 & Target Score & $\mathbf{91.845_{\pm 28.421}}$ & $\mathbf{-8.977_{\pm 1.433}}$ & $\mathbf{-9.984_{\pm 1.533}}$ & $-8.978_{\pm 1.434}$ & $\mathbf{0.671_{\pm 0.419}}$ & $0.617_{\pm 0.049}$ & $0.475_{\pm 0.132}$ & $0.044_{\pm 0.073}$ \\ 

\midrule

$0.5$ &  \no &  --- & \cellcolor{highlightorange} Target Score & $67.657_{\pm 11.985}$ & $-7.667_{\pm 0.687}$ & $-8.377_{\pm 0.661}$ & $-7.986_{\pm 0.948}$ & $0.251_{\pm 0.199}$ & $0.886_{\pm 0.006}$ & $\mathbf{0.969_{\pm 0.062}}$ & $0.244_{\pm 0.161}$  \\ 

$0.5$ &  \no &  --- & \cellcolor{highlightorange} Tempered Noise & $\mathbf{71.606_{\pm 15.139}}$ & $\mathbf{-7.838_{\pm 0.872}}$ & $\mathbf{-8.727_{\pm 0.878}}$ & $\mathbf{-8.085_{\pm 1.088}}$ & $\mathbf{0.362_{\pm 0.274}}$ & $\mathbf{0.887_{\pm 0.007}}$ & $0.944_{\pm 0.098}$ & $\mathbf{0.300_{\pm 0.212}}$ \\ 

\midrule

$0.5$ &  \yes &  $0.6$ & \cellcolor{highlightorange} Target Score & $77.100_{\pm 16.533}$ & $-8.243_{\pm 0.949}$ & $-9.112_{\pm 0.898}$ & $-8.337_{\pm 1.045}$ & $0.417_{\pm 0.337}$ & $0.877_{\pm 0.008}$ & $\mathbf{0.975_{\pm 0.023}}$ & $0.212_{\pm 0.155}$\\

$0.5$ &  \yes &  $0.6$ & \cellcolor{highlightorange} Tempered Noise & $\mathbf{78.501_{\pm 15.383}}$ & $\mathbf{-8.323_{\pm 0.919}}$ & $\mathbf{-9.127_{\pm 0.770}}$ & $\mathbf{-8.496_{\pm 1.100}}$ & $\mathbf{0.496_{\pm 0.308}}$ & $\mathbf{0.879_{\pm 0.016}}$ & $0.931_{\pm 0.064}$ & $\mathbf{0.250_{\pm 0.163}}$\\
\midrule
$2.0$ &  \no &  --- & \cellcolor{highlightorange} Target Score & $75.551_{\pm 16.345}$ & $\mathbf{-8.089_{\pm 0.899}}$ & $-8.966_{\pm 0.884}$ & $-8.309_{\pm 1.112}$ & $0.391_{\pm 0.331}$ & $\mathbf{0.881_{\pm 0.011}}$ & $\mathbf{0.994_{\pm 0.012}}$ & $\mathbf{0.288_{\pm 0.179}}$ \\ 

$2.0$ &  \no &  --- & \cellcolor{highlightorange} Tempered Noise & $\mathbf{75.868_{\pm 16.154}}$ & $-8.045_{\pm 0.909}$ & $\mathbf{-8.977_{\pm 0.978}}$ & $\mathbf{-8.352_{\pm 1.095}}$ & $\mathbf{0.460_{\pm 0.390}}$ & $0.874_{\pm 0.008}$ & $\mathbf{0.994_{\pm 0.012}}$ & $0.262_{\pm 0.186}$ \\ 

\midrule
$2.0$ &  \yes &  $0.6$ & \cellcolor{highlightorange} Target Score & $\mathbf{87.983_{\pm 22.856}}$ & $\mathbf{-8.790_{\pm 1.231}}$ & $\mathbf{-9.619_{\pm 1.101}}$ & $\mathbf{-8.988_{\pm 1.442}}$ & $\mathbf{0.569_{\pm 0.468}}$ & $\mathbf{0.818_{\pm 0.011}}$ & $\mathbf{0.888_{\pm 0.073}}$ & $0.212_{\pm 0.223}$ \\ 

$2.0$ &  \yes &  $0.6$ & \cellcolor{highlightorange} Tempered Noise & $79.696_{\pm 18.087}$ & $-8.229_{\pm 0.997}$ & $-9.104_{\pm 0.921}$ & $-8.681_{\pm 1.481}$ & $0.464_{\pm 0.429}$ & $0.796_{\pm 0.038}$ & $0.838_{\pm 0.109}$ & $\mathbf{0.331_{\pm 0.274}}$ \\ 

\midrule
$2.0$ &  \yes &  $0.7$ & \cellcolor{highlightorange} Target Score & $\mathbf{85.168_{\pm 21.258}}$ & $\mathbf{-8.574_{\pm 1.097}}$ & $-9.514_{\pm 1.028}$ & $\mathbf{-8.827_{\pm 1.452}}$ & $\mathbf{0.593_{\pm 0.484}}$ & $0.786_{\pm 0.034}$ & $0.806_{\pm 0.096}$ & $0.231_{\pm 0.224}$ \\ 

$2.0$ &  \yes &  $0.7$ & \cellcolor{highlightorange} Tempered Noise & $84.969_{\pm 18.906}$ & $-8.531_{\pm 0.980}$ & $\mathbf{-9.809_{\pm 1.170}}$ & $-8.545_{\pm 0.991}$ & $0.589_{\pm 0.427}$ & $\mathbf{0.796_{\pm 0.035}}$ & $\mathbf{0.850_{\pm 0.121}}$ & $\mathbf{0.262_{\pm 0.154}}$\\ 

     \bottomrule
\end{tabular}
}
\label{tab:dualtarget_ablation}
\end{table*}

==> tables/sdxl_metrics.tex <==
\begin{table}[ht]
\caption{Image generation using SDXL with classifier-free guidance (CFG). For all metrics mean values are reported.} 
\centering
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
$\beta$ & FKC & CLIP & ImageReward & Human Eval \\
\midrule
$2.5$ & \no & $33.89$ & $0.25$ & $4.85$\\
$7.5$ & \no & $\mathbf{36.00}$ & $0.74$ & $6.15$\\
$2.5$ & \yes & $35.87$ & $\mathbf{0.79}$ & $\mathbf{6.73}$ \\
\bottomrule
\end{tabular}%
}
\label{tab:sdxl_results}
\end{table}

==> text/DDPM_conversion.tex <==
\section{Implementation Details}

\subsection{Reformulating the DDPM backward diffusion process as a VP SDE}

We have $i = 0,\ldots,N$, with $q_{i=0}(x)$ the density of the data distribution
\begin{align}
    q_i(x_i\cond x_{i-1}) = \Normal(x_i \cond \sqrt{1-\beta_i} x_{i-1}, \beta_i)\,,\;\;
    x_i = \sqrt{1-\beta_i} x_{i-1} + \sqrt{\beta_i}\eps\,,\;\;\eps\sim\Normal(0,1)\,,
\end{align}
let's introduce other variables $\hat{x}_{i/N} = x_{i}$ and $\hat{\beta}_{i/N} = N\beta_{i}$
\begin{align}
    x_i =~& \sqrt{1-\frac{N\beta_i}{N}} x_{i-1} + \sqrt{\frac{N\beta_i}{N}}\eps\\
    \hat{x}_{i/N} =~& \sqrt{1-\frac{\hat{\beta}_{i/N}}{N}} \hat{x}_{(i-1)/N} + \sqrt{\frac{\hat{\beta}_{i/N}}{N}}\eps\\
    \hat{x}_{t+dt} =~& \sqrt{1-\hat{\beta}_{t+dt}dt} \hat{x}_{t} + \sqrt{\hat{\beta}_{t+dt}dt}\eps\\
    \hat{x}_{t+dt} =~& \left(1-\frac{1}{2}\hat{\beta}_{t+dt}dt\right) \hat{x}_{t} + \sqrt{\hat{\beta}_{t+dt}dt}\eps\\
    d\hat{x}_t =~& -\frac{1}{2}\hat{\beta}_t \hat{x}_tdt + \sqrt{\hat{\beta}_t}dW_t
\end{align}

\begin{align}
    \sqrt{1-\beta_3}\left(\sqrt{1-\beta_2}\left(\sqrt{1-\beta_1}x_0 + \sqrt{\beta_1}\eps_1\right) + \sqrt{\beta_2}\eps_2\right) + \sqrt{\beta_3}\eps_3
\end{align}
\begin{align}
    \beta_N + \sum_{i=1}^{N-1}\beta_i\prod_{j=i+1}^{N}(1-\beta_{j}) = 1-(1-\beta_N) + (1-\beta_N)\left(\beta_{N-1} + \sum_{i=1}^{N-2}\beta_i\prod_{j=i+1}^{N-1}(1-\beta_{j})\right)\\
    = 1 + (1-\beta_N)\left(\beta_{N-1} - 1 + \sum_{i=1}^{N-2}\beta_i\prod_{j=i+1}^{N-1}(1-\beta_{j})\right)\\
    = 1 + (1-\beta_N)\left(-(1-\beta_{N-1}) + (1-\beta_{N-1})\left(\beta_{N-2}+\sum_{i=1}^{N-3}\beta_i\prod_{j=i+1}^{N-2}(1-\beta_{j})\right)\right)\\
    = 1 + (1-\beta_N)(1-\beta_{N-1})\left(\beta_{N-2}-1 + \sum_{i=1}^{N-3}\beta_i\prod_{j=i+1}^{N-2}(1-\beta_{j})\right)\\
    = 1+ \prod_{i=3}^N (1-\beta_i)(\beta_2-1 + \beta_1(1-\beta_2))\\
    = 1+ \prod_{i=2}^N (1-\beta_i)(-1 + \beta_1)\\
    = 1- \prod_{i=1}^N (1-\beta_i)\\
\end{align}

Thus, the marginals are
\begin{align}
    q_i(x_i\cond x_0) = \Normal\left(x_i\cond \prod_{j=1}^i\sqrt{1-\beta_j}x_0, 1- \prod_{j=1}^i (1-\beta_j)\right)
\end{align}

\begin{align}
    q_t(x_t\cond x_0) = \Normal\left(x_t\cond \alpha_t x_0, \sigma_t^2\right)
\end{align}

\begin{align}
    \alpha_{i/N} = \prod_{j=1}^i\sqrt{1-\beta_j}\,,\;\;
    \sigma_{i/N}^2 = 1- \prod_{j=1}^i (1-\beta_j)
\end{align}

\begin{align}
    \alpha_{i/N} = \exp\left(\sum_{j=1}^i\log\sqrt{1-\beta_j}\right)\,,\;\;
    \sigma_{i/N}^2 = 1- \exp\left(\sum_{j=1}^i \log(1-\beta_j)\right)
\end{align}

\begin{align}
    \alpha_{i/N} = \exp\left(\frac{1}{2}\sum_{j=1}^i\log(1-\beta_j)\right)\,,\;\;
    \sigma_{i/N}^2 = 1- \exp\left(\sum_{j=1}^i \log(1-\beta_j)\right)
\end{align}

\begin{align}
    \beta_i = \frac{1}{N}\hat{\beta}\left(\frac{i}{N}\right)
\end{align}

==> text/algo.tex <==
\begin{algorithm}\label{algorithm:birth_death}
\caption{Outline of the Algorithm}
\begin{algorithmic}[1]
\STATE Sample initial states: ~ $\{ x_{t=0}^{(k)} \}_{k=1}^K \sim \meas_0$ 
\STATE Initialize log weights: ~  $ \{ w_{t=0}^{(k)} \}_{k=1}^K = 0$
\STATE Sample exponential clocks: ~ $\{ \tau^{(k)} \}_{k=1}^K \sim \text{Exponential}(1)$
\STATE Initialize excess/deficit:~ $\{ (w_{t=0}^{(k)})^+ \}_{k=1}^K = \{ (w_{t=0}^{(k)})^- \}_{k=1}^K =0$ 
% and $\{\lambda^{(k)}_{r:0}\}_{k=1}^K = 0$ 
%\STATE Initialize $\{r^{(k)} \}_{k=1}^K = 0$\COMMENT{indicating last reset time in index $k$}
\STATE \textbf{for} $t_i \in [t_1:t_T]$ \textbf{do}
\STATE \hspace{1em} $dt_i = t_i - t_{i-1}$
\STATE \hspace{1em} \textbf{for} $k \in [1:K]$ \textbf{do}
\STATE \hspace{2em} Simulate:~ $x_{t_i}^{(k)} = x_{t_{i-1}}^{(k)} + v_{{t_{i-1}}}(x_{t_{i-1}}^{(k)}) dt_i + \sigma_{t_{i-1}} \sqrt{dt_{i}}$  %\COMMENT{Simulate ODE/SDE for time $dt_i$}
%$\mathcal{L}^{*(v,\sigma)}_t[\mu_t^K](x_{t}^{(k)})$ via ODE/SDE for time $dt_i$
\STATE \hspace{2em} Increment weights:~  
$\Delta g_{t_i}^{(k)} = 
%w_{t_i}^{(k)} = w_{t_{i-1}}^{(k)} + 
g_{t_i}(x_{t_{i-1}}^{(k)}) dt_i$ %based on the specified PDE
\STATE \hspace{1em} 
%$\hat{w}_{t_i} = \frac{1}{K} \sum_{k=1}^K w_{t_i}^{(k)}$ 
$\Delta\hat{g}_{t_i} = \frac{1}{K} \sum_{k=1}^K \Delta g_{t_i}^{(k)}$
\STATE \hspace{1em} \textbf{for} $k \in [1:K]$ \textbf{do}
\STATE \hspace{2em} $(w_{t_i}^{(k)})^+ = (w_{t_{i-1}}^{(k)})^+ + dt_i
%\left( w_{t_i}^{(k)} - \hat{w}_{t_i} \right)^+$
\left( \Delta g_{t_i}^{(k)} - \Delta \hat{g}_{t_i}\right)^+$
\STATE \hspace{2em} $(w_{t_i}^{(k)})^- = (w_{t_{i-1}}^{(k)})^- + dt_i 
%\left( w_{t_i}^{(k)} - \hat{w}_{t_i} \right)^-$
\left( \Delta g_{t_i}^{(k)} - \Delta \hat{g}_{t_i}\right)^-$
\STATE \hspace{2em} \hlr{increment excess only (?)}
\STATE \hspace{2em} \textbf{if} $ (w_{t_i}^{(k)})^- \geq \tau^{(k)} $ \textbf{then}: 
\STATE \hspace{3em} Sample $\ell \sim \text{Categorical}\left(\left\{\dfrac{(w_{t_i}^{(\kappa)})^+}{\sum_{j=1}^K (w_{t_i}^{(j)})^+}\right\}_{\kappa=1}^{K}\right) $
\STATE \hspace{3em} \hlr{Note, this is based on threhsolding of accumulated excess, not $g_{t_i}^{(\kappa)}$}
\STATE \hspace{3em} Replace $x_{t_i}^{(k)} \gets x_{t_i}^{(\ell)}$
\STATE \hspace{3em} Sample new clock: ~ $\tau^{(k)} \sim \text{Exponential}(1)$
\STATE \hspace{3em} Reset weights: ~ $
%w_{t_i}^{(k)} = 
(w_{t_i}^{(k)})^+ =(w_{t_i}^{(k)})^- = 0$
%$k \in [1:K]$ \textbf{do}
\STATE \hspace{3em} \hlr{Reset cloned weights: $
%w_{t_i}^{(\ell)} = 
(w_{t_i}^{(\ell)})^+ =(w_{t_i}^{(\ell)})^- = 0$ }
\STATE \hspace{3em} \hlr{Without this step, we would never reset the accumulated excess weights $(w_{t_i})^+$}
\end{algorithmic}
\end{algorithm}
